Ontology Design Facilitating Wikibase Integration -- and a Worked Example for Historical Data

Wikibase -- which is the software underlying Wikidata -- is a powerful platform for knowledge graph creation and management. However, it has been developed with a crowd-sourced knowledge graph creation scenario in mind, which in particular means that it has not been designed for use case scenarios in which a tightly controlled high-quality schema, in the form of an ontology, is to be imposed, and indeed, independently developed ontologies do not necessarily map seamlessly to the Wikibase approach. In this paper, we provide the key ingredients needed in order to combine traditional ontology modeling with use of the Wikibase platform, namely a set of \emph{axiom} patterns that bridge the paradigm gap, together with usage instructions and a worked example for historical data.

==> axiomatization_scratch.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Axiomatization}
\label{ssec:axioms}
%%%%%
% What is the purpose of the axiomatization?
The overarching purpose of this axiomatization is to be able to conceptually reason about the modules. The axiomatization shall capture statements such as the following.
\begin{compactenum}
    \item "There is always a qualifier for"
    \item "The qualifier needs to be a certain type"
\end{compactenum}
Recall that \textsf{propertyName}, \textsf{qualifierName}, and \textsf{referenceName} are \emph{placeholders} to improve the clarity of these diagrams. They are meant to be replaced when utilizing these patterns and their expansions. Indeed, when replacing one, the corresponding occurrences will all be replaced by the same predicate name, and they will then be distinguishable by their namespaces.

For example, we may replace \textsf{wdt:propertyName} with \textsf{wdt:hasName} and have the edge point to an \textsf{xsd:string}. At that point, we would replace all instances of ``propertyName'' with ``hasName'' across all namespaces in the diagram. We would then use Figure~\ref{fig:state-s} and the accompanying axiomatization. Additional examples can be found in Section~\ref{sec:example}.

% What's in this section?
In the following sections, we provide the description logic formulation of the axioms.\footnote{Additional information on the syntax and construction can be found in \cite{FOST,dl-primer}.}
% Shortened Prexies
We have shortened some prefixes and predicates due to length: \textsf{wikibase:} has been shortened to \textsf{wb:}, \textsf{referenceName} to \textsf{refName}, \textsf{propertyName} to \textsf{propName}, and \textsf{wasDerivedFrom} to \textsf{wDF}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Figures
\begin{figure}[tb]
    \centering
    \includegraphics[width=\columnwidth]{figures/patterns/pattern-generic}
    \caption{The top diagram shows a condensed view of the wikibase conceptual model. The bottom diagram shows how the \emph{expansion} of the diagram to include the nodes that are automatically generated by the wikibase framework. We use a diamond arrowhead and orange color to denote \textsf{Qualifier} nodes. A circle arrowhead and blue color to denote \textsf{Reference} nodes. In the expanded diagrams (in the lower portion), we change the border color of the nodes to indicate the origin of the generated nodes.}
    \label{fig:pattern-generic}
\end{figure}
\begin{figure}[tb]
    \centering
    \includegraphics[width=\columnwidth]{figures/patterns/qualifier-datetime.jpg}
    \caption{Condensed (top) and expanded (bottom) schema diagrams with an \textsf{xsd:datetime} for a qualifer. Nodes bordered in orange expand from the label node in the top diagram.}
    \label{fig:qual-dt}
\end{figure}
\begin{figure}[tb]
    \centering
    \includegraphics[width=\columnwidth]{figures/patterns/qualifier-quantity.jpg}
    \caption{Condensed (top) and expanded (bottom) schema diagrams for modeling with \textsf{xsd:decimal} as a qualifer to \textsf{wdt:propertyName}.}
    \label{fig:qual-q}
\end{figure}
\begin{figure}[tb]
    \centering
    \includegraphics[width=\columnwidth]{figures/patterns/qualifier-string.jpg}
    \caption{Condensed (top) and expanded (bottom) schema diagrams for modeling with \textsf{xsd:string} as a qualifer for \textsf{wdt:propertyName}.}
    \label{fig:qual-s}
\end{figure}
\begin{figure}[tb]
    \centering
    \includegraphics[width=\columnwidth]{figures/patterns/ref-without-qualifier.jpg}
    \caption{Condensed (top) and expanded (bottom) schema diagrams including a Reference for the assertions made by \textsf{wdt:propertyName}.}
    \label{fig:ref-nq}
\end{figure}
\begin{figure}[tb]
    \centering
    \includegraphics[width=\columnwidth]{figures/patterns/statement-datetime.jpg}
    \caption{Condensed (top) and expanded (bottom) schema diagrams when modeling \textsf{wdt:propertyName} as a data property and the datatype is a \textsf{xsd:datetime}.}
    \label{fig:state-dt}
\end{figure}
\begin{figure}[tb]
    \centering
    \includegraphics[width=\columnwidth]{figures/patterns/statement-quanity.jpg}
    \caption{Condensed (top) and expanded (bottom) schema diagrams when modeling \textsf{wdt:propertyName} as a data property and the datatype is a \textsf{xsd:decimal}.}
    \label{fig:state-q}
\end{figure}
\begin{figure}[tb]
    \centering
    \includegraphics[width=.7\columnwidth]{figures/patterns/statement-string.jpg}
    \caption{Condensed (top) and expanded (bottom) schema diagrams when modeling \textsf{wdt:propertyName} as a data property and the datatype is a \textsf{xsd:string}.}
    \label{fig:state-s}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Axioms Invariant to Expansion Type}
\label{sssec:invariant}
%%%%%
In this section, we discuss those axioms that appear to be invariant under the expansion type, as seen in Figure~\ref{fig:pattern-generic}.
%%%%%
\begin{align}
    % (Axiom 1) p:propertyName domain -> ?
    \exists ~\textsf{p:propName}.\top &\sqsubseteq \textsf{wb:Item} \\
    % (Axiom 2) p:propertyName range -> wikibase:Statement
    \top &\sqsubseteq \phantom{\mathord{\leq}}\forall~\textsf{p:propName.wb:Statement} \\
    % (Axiom 3) p:propertyName inverse functional
    \top &\sqsubseteq \mathord{\leq}1~\textsf{p:propName}^-\textsf{.wb:Statement} \\
    % (Axiom 4) p:propertyName inverse existential
    \top &\sqsubseteq \phantom{\mathord{\leq}}\exists~\textsf{p:propName}^-\textsf{.wb:Statement}
\end{align}
% Axiom 1
Axiom 1 is a domain restriction. That is, the inverse filler (i.e., the domain) is restricted to \textsf{wb:Item}. 
% Axiom 2
Axiom 2 is a range restriction. That is, the filler (i.e., the range) is restricted to \textsf{wb:Statement}.
% Axiom 3
Axiom 3 states that \textsf{p:propName} is inverse functional. That is, a particular hashed statement node is the target of at most one \textsf{wb:Item} via \textsf{p:propName}.
% Axiom 4
Axiom 4 then states that \textsf{p:propName} is also inverse existential. This means that there always exists some \textsf{wb:Item} that is the inverse filler for \textsf{p:propName}. Together with Axioms 1 and 3, this indicates that any particular \textsf{wb:Statement} node is not orphaned. That is, a \textsf{wb:Statement} node is always the filler for \textsf{p:propName} with a \textsf{wb:Item} as the inverse filler.
\begin{align}
    % (Axiom 5) ps:propertyName domain -> wikibase:Statement
    \exists ~\textsf{ps:propName}.\top &\sqsubseteq \textsf{wb:Statement} \\
    % (Axiom 6) ps:propertyName range -> wikibase:Item
\top &\sqsubseteq \phantom{\mathord{\leq}}\forall~\textsf{p:propName.wb:Item} \\
    % (Axiom 7) ps:propertyName functional
    \top &\sqsubseteq \mathord{\leq}1~\textsf{ps:propName.wb:Item} \\
    % (Axiom 8) ps:propertyName existential
    \top &\sqsubseteq \phantom{\mathord{\leq}}\exists~\textsf{ps:propName.wb:Item}
\end{align}
% Axiom 5
Axiom 5 is a domain restriction. That is, the inverse filler (i.e., the domain) is restricted to \textsf{wb:Statement}.
% Axiom 6
Axiom 6 is a range restriction. That is, the filler (i.e., the range) is restricted to \textsf{wb:Item}.
% Axiom 7
Axiom 7 states that \textsf{ps:propName} is functional. That is, a particular hashed statement node targets at most one \textsf{wb:Item} via \textsf{ps:propName}.
% Axiom 8
Axiom 8 then states that \textsf{ps:propName} is also existential. This means that there always exists some \textsf{wb:Item} that is a filler for \textsf{ps:propName} for every \textsf{wb:Statement}.
\begin{align}
    % (Axiom 9) pq:qualifierName domain -> wikibaseStatement
    \exists ~\textsf{pq:qualifierName}.\top &\sqsubseteq \textsf{wb:Statement}
    % Can't really say more than this, here.
\end{align}
% Axiom 9
Axiom 9 states that the domain of a \textsf{pq:qualifierName} relation is always a \textsf{wb:Statement}.
% Can't say more.
Additional restrictions on this property depend on the type of qualifier in question. These are examined in the next sections.
\begin{align}
    % (Axiom 10) prov:wasDerivedFrom domain -> wikibase:Statement
    \exists ~\textsf{prov:wDF.}\top &\sqsubseteq \textsf{wb:Statement} \\
    % (Axiom 11) prov:wasDerivedFrom range -> wikibase:Reference
    \top &\sqsubseteq \forall~\textsf{prov:wDF.wb:Reference} \\
    % (Axiom 12) prov:wasDerivedFrom inverse functional
    \textsf{wb:Reference} &\sqsubseteq \exists~\textsf{prov:wDF}^-.\top \\
    % (Axiom 13) pr:referenceName domain -> wikibase:Reference
    \exists ~\textsf{pr:refName.}\top &\sqsubseteq \textsf{wb:Reference}
\end{align}
% Axiom 10
Axiom 10 is a domain restriction. That is, the inverse filler (i.e., the domain) of \textsf{prov:wDF} is restricted to \textsf{wb:Statement}.
% Axiom 11
Axiom 11 is a range restriction. That is, the filler (i.e., the range) of \textsf{prov:wDF} is restricted to \textsf{wb:Reference}.
% Axiom 12
Axiom 12 states that \textsf{prov:wasDF} is inverse functional. That is, a particular hashed reference node is the target of at most one \textsf{wb:Statement} via \textsf{prov:wDF}.
% Axiom 13
Axiom 13 is a domain restriction. That is, the inverse filler (i.e., the domain) of \textsf{pr:referenceName} is a \textsf{wb:Item}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Axioms for Relations Between Items}
\label{sssec:ax-item}
%%%%%
\begin{align}
    % (Axiom 14) p:propertyName o ps:propertyName $\sqsubseteq$ wdt:propertyName
    \textsf{p:propName} \circ \textsf{ps:propName} &\sqsubseteq \textsf{wdt:propName}
\end{align}
% Axiom 14
Axiom 14 is a role chain that connects \textsf{wb:Items} via the reified \textsf{wb:Statement} node.
\begin{align}
    % (Axiom 15) wdt:propertyName domain -> wb:Item (same as p:propertyName)
    \exists~\textsf{wdt:propName}.\top &\sqsubseteq \textsf{wb:Item} \\
    % (Axiom 16) wdt:propertyName scoped domain -> wb:Item (can be expressed over role chain?)
    \exists~\textsf{wdt:propName.wb:Item} &\sqsubseteq \textsf{wb:Item}
\end{align}
% Axiom 15
Axiom 15 is a domain restriction. That is, the inverse filler (i.e., the domain) of \textsf{wdt:propName} is restricted to \textsf{wb:Item}.
% Axiom 16
Axiom 16 is a scoped domain restriction. That is, when the filler (i.e., the range) is of type \textsf{wb:Item}, the inverse filler (i.e., the domain) of \textsf{prov:wDF} is restricted to \textsf{wb:Item}.
\begin{align}
    % (Axiom 17) wdt:propertyName range -> wb:Item (same as ps:propertyName)
    \exists~\textsf{wdt:propName}^-.\top &\sqsubseteq \textsf{wb:Item} \\
    % (Axiom 18) wdt:propertyName scoped range -> wb:Item (can not be expressed over role chain?)
    \exists~\textsf{wdt:propName}^-\textsf{wb:Item} &\sqsubseteq \textsf{wb:item}
\end{align}
% Axiom 17
Axiom 17 is a range restriction and 
% Axiom 18
Axiom 18 is a scoped range restriction. These is accomplished using \emph{inverse domain restrictions} to avoid the use of a complex predicate (i.e., the role chain from Axiom 14) on the right-hand side of the axiom in order to keep the axiomatization within OWL 2.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Axioms for Qualifiers}
\label{sssec:ax-qual}
%%%%%
These axiomatizations pertain to Figures~\ref{fig:qual-dt}-\ref{fig:qual-s}. 
% Think: natural language things we may want to say about the qualifier, and how they are reflected as axioms on the expanded version.
The expansion of a particular qualifier changes depending on the type of qualifier. That is, Wikibase creates different sets of triples when the qualifier is a string versus a datetime, and so on. This restriction can be specified, in general, as follows, as a rule.
\begin{align*}
    \forall x,y,z ~\textsf{Item}(x)~&\wedge~\textsf{p:propName}(x,y)~\notag\\&\wedge~\textsf{pq:qualName}(y,z)~\longrightarrow~\textsf{Qualifier}(z)
\end{align*}
Where \textsf{Qualifier} is the type of the particular qualifier (e.g., \textsf{xsd:string}).
% Axioms 19 and 20
We can specify this in description logic as complex inverse scoped domain restriction, as in Axiom 19. Similarly, in Axiom 20, we also wish to constrain \textsf{pq:qualName} to be functional, dependent on type.
\begin{align}
    % Axiom 19 (range restriction on type of qualifier for a type)
    \exists~\textsf{pq:qualName}^-.\left(\exists~\textsf{p:propName}^-\textsf{.Item}\right) &\sqsubseteq \textsf{Qualifier} \\
    % Axiom 20 (functionality on qualifiers)
    \exists~\textsf{pq:qualName}^-.\left(\exists~\textsf{p:propName}^-\textsf{.Item}\right) &\sqsubseteq \textsf{Qualifier}
\end{align}
Finally, in some cases, we may want to say that certain statements always have a qualifier of a certain type. This can be expressed as in Axiom 21.
\begin{align}
    % Axiom 21 (require a qualifier of a certain type)
    \exists~\textsf{pq:qualName}^-.\left(\exists~\textsf{p:propName}^-\textsf{.Item}\right) &\sqsubseteq \textsf{Qualifier}
\end{align}

% inverse functionality -- how to word this in natural language?
% I don't think we can actually do this, as qualifiers are datatypes

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Qualifying with a date}
\label{sssec:ax-qual-dt}
%%%%%
Wikibase uses \textsf{xsd:dateTime} for this purpose. The pattern for using \textsf{xsd:dateTime} as a qualifier can be found in Figure~\ref{fig:qual-dt}.
% pq:qualName
\begin{align}
  % scoped domain restriction
  \exists~\textsf{pq:qualName.xsd:dateTime} &\sqsubseteq \textsf{wb:Statement}  \label{ax:qn-sd-dt}
\end{align}
% Axiom
Axiom \ref{ax:qn-sd-dt} is a scoped domain restriction. That is, when the filler (i.e., the range) is of type \textsf{xsd:dateTime}, the inverse filler (i.e., the domain) of \textsf{pq:qualName} is restricted to \textsf{wb:Statement}.
\begin{align}
  % scoped range restriction
  \textsf{wb:Statement} &\sqsubseteq \forall~\textsf{pq:qualName.xsd:dateTime}  \label{ax:qn-sr-dt}\\
  % functional
  \textsf{wb:Statement} &\sqsubseteq \mathord{\leq}1~\textsf{pq:qualName.xsd:dateTime}  \label{ax:qn-f-dt}
\end{align}
% Axiom
Axiom \ref{ax:qn-sr-dt} is a scoped range restriction. That is, when the inverse filler (i.e., the domain) is of type \textsf{wb:Statement}, the filler (i.e., the range) of \textsf{pq:qualName} is restricted to \textsf{xsd:dateTime}.
% Axiom
Axiom \ref{ax:qn-f-dt} states that \textsf{pq:qualName} is functional. That is, a particular \textsf{wb:Statement} node targets at most one \textsf{xsd:dateTime} via \textsf{pq:qualName}.

% pqv:qualName
\begin{align}
  % domain restriction
  \exists~\textsf{pqv:qualName.}\top &\sqsubseteq \textsf{wb:Statement}  \label{ax:qn-d}\\
  % scoped range restriction
  \textsf{wb:Statement} &\sqsubseteq \forall~\textsf{pqv:qualName.wb:QuantityValue}  \label{ax:qn-sr}\\
  % functional
  \textsf{wb:Statement} &\sqsubseteq \mathord{\leq}1~\textsf{pqv:qualName.wb:QuantityValue}  \label{ax:qn-f}
\end{align}
% Axiom
Axiom \ref{ax:qn-d} is a domain restriction. That is, the inverse filler (i.e., the domain) is restricted to \textsf{wb:Statement}.
% Axiom
Axiom \ref{ax:qn-sr} is a scoped range restriction. That is, when the inverse filler (i.e., the domain) is of type \textsf{wb:Statement}, the filler (i.e., the range) of \textsf{pqv:qualName} is restricted to \textsf{wb:QuantityValue}.
% Axiom
Axiom \ref{ax:qn-f} states that \textsf{pqv:qualName} is functional. That is, a particular \textsf{wb:Statement} node targets at most one \textsf{wb:QuantityValue} via \textsf{pqv:qualName}.

% wb:quantityValue
\begin{align}
  % domain restriction
  \exists~\textsf{wb:quantityValue.}\top &\sqsubseteq \textsf{wb:QuantityValue}  \label{ax:qv-d}\\
  % scoped range restriction
  \textsf{wb:QuantityValue} &\sqsubseteq \forall~\textsf{wb:quantityValue.xsd:decimal}  \label{ax:qv-sr}\\
  % existential
  \textsf{wb:QuantityValue} &\sqsubseteq \exists~\textsf{wb:quantityValue.wb:QuantityValue}  \label{ax:qv-e}\\
  % functional
  \textsf{wb:QuantityValue} &\sqsubseteq \mathord{\leq}1~\textsf{wb:quantityValue.xsd:decimal}  \label{ax:qv-f}
\end{align}
% Axiom
Axiom \ref{ax:qv-d} is a domain restriction. That is, the inverse filler (i.e., the domain) is restricted to \textsf{wb:QuantityValue}.
% Axiom
Axiom \ref{ax:qv-sr} is a scoped range restriction. That is, when the inverse filler (i.e., the domain) is of type \textsf{wb:QuantityValue}, the filler (i.e., the range) of \textsf{wb:quantityValue} is restricted to \textsf{xsd:decimal}.
% Axiom
Axiom \ref{ax:qv-e} states that \textsf{wb:quantityValue} is existential. That is \placeholder{}
% Axiom
Axiom \ref{ax:qv-f} states that \textsf{wb:quantityValue} is functional. That is, a particular \textsf{wb:QuantityValue} node targets at most one \textsf{xsd:decimal} via \textsf{wb:quantityValue}.

% wb:quantityUnit
\begin{align}
  % domain restriction
  \exists~\textsf{wb:quantityUnit.}\top &\sqsubseteq \textsf{wb:QuantityValue}  \label{ax:qu-d}\\
  % scoped range restriction
  \textsf{wb:QuantityValue} &\sqsubseteq \forall~\textsf{wb:quantityUnit.wb:Item}  \label{ax:qu-sr}\\
  % existential
  \textsf{wb:QuantityValue} &\sqsubseteq \exists~\textsf{wb:quantityUnit.wb:QuantityValue}  \label{ax:qu-e}\\
  % functional
  \textsf{wb:QuantityValue} &\sqsubseteq \mathord{\leq}1~\textsf{wb:quantityUnit.wb:Item}  \label{ax:qu-f}
\end{align}
% Axiom
Axiom \ref{ax:qu-d} is a domain restriction. That is, the inverse filler (i.e., the domain) is restricted to \textsf{wb:QuantityValue}.
% Axiom
Axiom \ref{ax:qu-sr} is a scoped range restriction. That is, when the inverse filler (i.e., the domain) is of type \textsf{wb:QuantityValue}, the filler (i.e., the range) of \textsf{wb:quantityUnit} is restricted to \textsf{wb:Item}.
% Axiom
Axiom \ref{ax:qu-e} states that \textsf{wb:quantityUnit} is existential. That is \placeholder{}
% Axiom
Axiom \ref{ax:qu-f} states that \textsf{wb:quantityUnit} is functional. That is, a particular \textsf{wb:QuantityValue} node targets at most one \textsf{wb:Item} via \textsf{wb:quantityUnit}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Qualifying with a quantity}
\label{sssec:ax-qual-q}
%%%%%
Wikibase uses \textsf{xsd:decimal} with \textsf{wikibase:QuantityUnit} for this purpose.
The pattern for using \textsf{xsd:decimal} as a qualifier can be found in Figure~\ref{fig:qual-q}. Qualifying with a quantity creates a construction that incorporates the unit of the quantity, which is also a \textsf{wb:Item}. It does this by creating another hash node of type \textsf{wb:QuantityValue}, this time in the \textsf{v:} namespace. The hashnode is referenced with \textsf{qualName} as well, but in the \textsf{pqv:} namespace. \textsf{pq:qualName} still points directly to the amount itself.
% pq:qualName
\begin{align}
  % domain restriction
  \exists~\textsf{pq:qualName.}\top &\sqsubseteq \textsf{wb:Statement}  \label{ax:qn-d}\\
  % scoped range restriction
  \textsf{wb:Statement} &\sqsubseteq \forall~\textsf{pq:qualName.xsd:decimal}  \label{ax:qn-sr}\\
  % functional
  \textsf{wb:Statement} &\sqsubseteq \mathord{\leq}1~\textsf{pq:qualName.xsd:decimal}  \label{ax:qn-f}
\end{align}
% Axiom
Axiom \ref{ax:qn-d} is a domain restriction. That is, the inverse filler (i.e., the domain) is restricted to \textsf{wb:Statement}.
% Axiom
Axiom \ref{ax:qn-sr} is a scoped range restriction. That is, when the inverse filler (i.e., the domain) is of type \textsf{wb:Statement}, the filler (i.e., the range) of \textsf{pq:qualName} is restricted to \textsf{xsd:decimal}.
% Axiom
Axiom \ref{ax:qn-f} states that \textsf{pq:qualName} is functional. That is, a particular \textsf{wb:Statement} node targets at most one \textsf{xsd:decimal} via \textsf{pq:qualName}.

% pqv:qualName
\begin{align}
  % domain restriction
  \exists~\textsf{pqv:qualName.}\top &\sqsubseteq \textsf{wb:Statement}  \label{ax:qn-v-d}\\
  % scoped range restriction
  \textsf{wb:Statement} &\sqsubseteq \forall~\textsf{pqv:qualName.wb:QuantityValue}  \label{ax:qn-v-sr}\\
  % functional
  \textsf{wb:Statement} &\sqsubseteq \mathord{\leq}1~\textsf{pqv:qualName.wb:QuantityValue}  \label{ax:qn-v-f}
\end{align}
% Axiom
Axiom \ref{ax:qn-v-d} is a domain restriction. That is, the inverse filler (i.e., the domain) is restricted to \textsf{wb:Statement}.
% Axiom
Axiom \ref{ax:qn-v-sr} is a scoped range restriction. That is, when the inverse filler (i.e., the domain) is of type \textsf{wb:Statement}, the filler (i.e., the range) of \textsf{pqv:qualName} is restricted to \textsf{wb:QuantityValue}.
% Axiom
Axiom \ref{ax:qn-v-f} states that \textsf{pqv:qualName} is functional. That is, a particular \textsf{wb:Statement} node targets at most one \textsf{wb:QuantityValue} via \textsf{pqv:qualName}.

% wb:quantityValue
\begin{align}
  % domain restriction
  \exists~\textsf{wb:quantityValue.}\top &\sqsubseteq \textsf{wb:QuantityValue}  \label{ax:qv-d}\\
  % scoped range restriction
  \textsf{wb:QuantityValue} &\sqsubseteq \forall~\textsf{wb:quantityValue.xsd:decimal}  \label{ax:qv-sr}\\
  % existential
  \textsf{wb:QuantityValue} &\sqsubseteq \exists~\textsf{wb:quantityValue.wb:QuantityValue}  \label{ax:qv-e}\\
  % functional
  \textsf{wb:QuantityValue} &\sqsubseteq \mathord{\leq}1~\textsf{wb:quantityValue.xsd:decimal}  \label{ax:qv-f}
\end{align}
% Axiom
Axiom \ref{ax:qv-d} is a domain restriction. That is, the inverse filler (i.e., the domain) is restricted to \textsf{wb:QuantityValue}.
% Axiom
Axiom \ref{ax:qv-sr} is a scoped range restriction. That is, when the inverse filler (i.e., the domain) is of type \textsf{wb:QuantityValue}, the filler (i.e., the range) of \textsf{wb:quantityValue} is restricted to \textsf{xsd:decimal}.
% Axiom
Axiom \ref{ax:qv-e} states that \textsf{wb:quantityValue} is existential. That is \placeholder{}
% Axiom
Axiom \ref{ax:qv-f} states that \textsf{wb:quantityValue} is functional. That is, a particular \textsf{wb:QuantityValue} node targets at most one \textsf{xsd:decimal} via \textsf{wb:quantityValue}.

% wb:quantityUnit
\begin{align}
  % domain restriction
  \exists~\textsf{wb:quantityUnit.}\top &\sqsubseteq \textsf{wb:QuantityValue}  \label{ax:qu-d}\\
  % scoped range restriction
  \textsf{wb:QuantityValue} &\sqsubseteq \forall~\textsf{wb:quantityUnit.wb:Item}  \label{ax:qu-sr}\\
  % existential
  \textsf{wb:QuantityValue} &\sqsubseteq \exists~\textsf{wb:quantityUnit.wb:QuantityValue}  \label{ax:qu-e}\\
  % functional
  \textsf{wb:QuantityValue} &\sqsubseteq \mathord{\leq}1~\textsf{wb:quantityUnit.wb:Item}  \label{ax:qu-f}
\end{align}
% Axiom
Axiom \ref{ax:qu-d} is a domain restriction. That is, the inverse filler (i.e., the domain) is restricted to \textsf{wb:QuantityValue}.
% Axiom
Axiom \ref{ax:qu-sr} is a scoped range restriction. That is, when the inverse filler (i.e., the domain) is of type \textsf{wb:QuantityValue}, the filler (i.e., the range) of \textsf{wb:quantityUnit} is restricted to \textsf{wb:Item}.
% Axiom
Axiom \ref{ax:qu-e} states that \textsf{wb:quantityUnit} is existential. That is \placeholder{}
% Axiom
Axiom \ref{ax:qu-f} states that \textsf{wb:quantityUnit} is functional. That is, a particular \textsf{wb:QuantityValue} node targets at most one \textsf{wb:Item} via \textsf{wb:quantityUnit}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Qualifying with a string}
\label{sssec:ax-qual-s}
%%%%
Wikibase uses \textsf{xsd:string} for this purpose.
The pattern for using \textsf{xsd:string} as a qualifier can be found in Figure~\ref{fig:qual-s}.
Qualifying with a string is very simple and consists of only the relation and value.
% pq:qualName
\begin{align}
  % domain restriction
  \exists~\textsf{pq:qualName.}\top &\sqsubseteq \textsf{wb:Statement}  \label{ax:qn-d}\\
  % range restriction
  \top &\sqsubseteq \forall~\textsf{pq:qualName.xsd:string}  \label{ax:qn-r}\\
  % functional
  \textsf{wb:Statement} &\sqsubseteq \mathord{\leq}1~\textsf{pq:qualName.xsd:string}  \label{ax:qn-f}
\end{align}
% Axiom
Axiom \ref{ax:qn-d} is a domain restriction. That is, the inverse filler (i.e., the domain) is restricted to \textsf{wb:Statement}.
% Axiom
Axiom \ref{ax:qn-r} is a range restriction. That is, the filler (i.e., the range) is restricted to \textsf{xsd:string}.
% Axiom
Axiom \ref{ax:qn-f} states that \textsf{pq:qualName} is functional. That is, a particular \textsf{wb:Statement} node targets at most one \textsf{xsd:string} via \textsf{pq:qualName}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Axioms for References}
\label{sssec:ax-refs}
%%%%%
Figure \ref{fig:ref-nq}.
% pr:referenceName
\begin{align}
  % domain restriction
  \exists~\textsf{pr:referenceName.}\top &\sqsubseteq \textsf{wb:Reference}  \label{ax:rn-d}\\
  % range restriction
  \top &\sqsubseteq \forall~\textsf{pr:referenceName.wb:Item}  \label{ax:rn-r}\\
  % existential
  \textsf{wb:Reference} &\sqsubseteq \exists~\textsf{pr:referenceName.wb:Reference}  \label{ax:rn-e}\\
  % functional
  \textsf{wb:Reference} &\sqsubseteq \mathord{\leq}1~\textsf{pr:referenceName.wb:Item}  \label{ax:rn-f}
\end{align}
% Axiom
Axiom \ref{ax:rn-d} is a domain restriction. That is, the inverse filler (i.e., the domain) is restricted to \textsf{wb:Reference}.
% Axiom
Axiom \ref{ax:rn-r} is a range restriction. That is, the filler (i.e., the range) is restricted to \textsf{wb:Item}.
% Axiom
Axiom \ref{ax:rn-e} states that \textsf{pr:referenceName} is existential. That is \placeholder{}
% Axiom
Axiom \ref{ax:rn-f} states that \textsf{pr:referenceName} is functional. That is, a particular \textsf{wb:Reference} node targets at most one \textsf{wb:Item} via \textsf{pr:referenceName}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Axioms for Statements}
%%%%%
Previously, we discussed when \textsf{wdt:propName} had a \textsf{wb:Item} as a filler. However, it is also possible to have fillers that are datatypes, in particular \textsf{xsd:datetime}, \textsf{xsd:decimal}, and \textsf{xsd:string}. These can be see in Figures~\ref{fig:state-dt}, \ref{fig:state-q}, and \ref{fig:state-s}. The axiomatizations of these diagrams follow as those presented in Sections \ref{sssec:ax-qual-dt}, \ref{sssec:ax-qual-q}, and \ref{sssec:ax-qual-s}, but use namespace \textsf{psv:} instead of \textsf{pqv:}.


